Convex Hierarchical Clustering for Graph-Structured Data

Convex clustering is a recent stable alternative to hierarchical clustering. It formulates the recovery of progressively coalescing clusters as a regularized convex problem. While convex clustering was originally designed for handling Euclidean distances between data points, in a growing number of applications, the data is directly characterized by a similarity matrix or weighted graph. In this paper, we extend the robust hierarchical clustering approach to these broader classes of similarities. Having defined an appropriate convex objective, the crux of this adaptation lies in our ability to provide: (a) an efficient recovery of the regularization path and (b) an empirical demonstration of the use of our method. We address the first challenge through a proximal dual algorithm, for which we characterize both the theoretical efficiency as well as the empirical performance on a set of experiments. Finally, we highlight the potential of our method by showing its application to several real-life datasets, thus providing a natural extension to the current scope of applications of convex clustering.

==> abstract.tex <==
% !TEX root = main.tex




%From gene sequencing to biomedical studies, hierarchical clustering has become one of the most popular procedures for data analysis across a wide number of disciplines. 
%Hierarchical clustering allows the discovery of natural groupings of the data at different scales by recovering progressively coalescing sequences of clusters. However, this inherently greedy optimization procedure is sensitive to both the choice of the linkage function and small perturbations of the dataset ---a considerable drawback in a number of applications where the robustness and generalization power of the clusters are prerequisites for the analysis. 
Convex clustering \cite{chi2017convex} is a recent stable alternative to hierarchical clustering which formulates the recovery of progressively coalescing clusters as a regularized convex problem. While convex clustering was originally designed for handling Euclidean distances between data points, in a growing number of applications, such Euclidean representations are not readily available. Rather, the data is directly characterized by a similarity matrix or weighted graph. In this paper, we  extend the robust hierarchical clustering approach to much broader classes of similarities. Having defined an appropriate convex objective, the crux of this adaptation lies in our ability to provide: (a) an efficient recovery of the regularization path and (b) an empirical demonstration of the use of our method.  We address the first challenge through a proximal dual algorithm for which we characterize both the theoretical efficiency and the empirical performance on a set of experiments. Finally, we highlight the potential of our method by showing its application to several real-life datasets, thus providing a natural extension to the current scope of applications of convex clustering.

lll
%Hierarchical clustering is an extensively-used procedurerecovers a nested sequence of clusters and their progressive fusions yields an intuitive and comprehensible summary of the data. However, current hierarchical clustering algorithms are inherently greedy-- making the recovered clusters and their coalescence path sensitive to both the choice of linkage function and the presence of outliers. Convex clustering has been recently proposed as an alternative for hierarchical clustering addressing these issues by solving a convex problem and recovering a solution with optimality guarantees.  However, most of the literature in convex clustering focuses on feature-valued vectors. Yet, in a number of applications, such feature vectors are not readily available and the data comes directly in the form of a similarity matrix between data points. In this paper, we propose to tackle this problem by deriving a convex equivalent of hierarchical clustering for graph data. We derive a fast algorithm for solving this convex problem, and evaluate the performance of the method on several datasets. 

==> synthetic_exp.tex <==
% !TEX root = pooling_nips_2018.tex





To assess the performance of our method, we begin by a set of synthetic experiment. We generate a three layer hierarchical graph, where each level.



